PU-Net: Point Cloud Upsampling Network

Learning and analyzing 3D point clouds with deep networks is challenging due to the sparseness and irregularity of the data. In this paper, we present a data-driven point cloud upsampling technique. The key idea is to learn multi-level features per point and expand the point set via a multi-branch convolution unit implicitly in feature space. The expanded feature is then split to a multitude of features, which are then reconstructed to an upsampled point set. Our network is applied at a patch-level, with a joint loss function that encourages the upsampled points to remain on the underlying surface with a uniform distribution. We conduct various experiments using synthesis and scan data to evaluate our method and demonstrate its superiority over some baseline methods and an optimization-based method. Results show that our upsampled points have better uniformity and are located closer to the underlying surfaces.

==> dataset.tex <==
\subsection{Datasets}
To make our training dataset more diverse, we collect 40 different meshes from Visionair repository~\cite{timmurphy.org} ranging from simple, smooth models to complex steep models.
We cut 100 patches with various patch size from each model.
Therefore, the size of training dataset is 4000.

In the test phase, there are two kinds of different dataset.
\begin{itemize}	
	\item
	Our collected models: We download another 20 models from the above Visionair repository that are different from those training models.
	\item
	SHREC15: There are 1200 shapes from 50 categories. From each category, we randomly choose one model. Thus, totally 50 models for test.
\end{itemize}
For more testing results on ModelNet and ShapeNet dataset, please refer to our supplementary material.

==> relatedwork.tex <==
\section{Related Work}

\phil{TODO: 1) please survey and add papers on point cloud processing and upsampling in graphics and geometry (without deep learning), e.g., PCL; 2) point set or point cloude processing with deep learning... these are two areas that are most related to our work; apart from them, any other topic else?}

In this section, we give a brief review of previous works that are most related with our paper.
We first review geometric approaches for upsampling that are commonly used for surface reconstruction or point-based rendering.
Finally, we provide a picture for deep learning-based point cloud processing.

\para{Geometric approaches for upsampling} \ \ \ Early work by Alexa et al.~\cite{alexa2003computing} proposed to upsample a point set via interpolating points at vertices of a Voronoi diagrams in local tangent spaces, which is used for point set rendering.
Lipman et al.~\cite{lipman2007parameterization} presented a locally optimal projection (LOP) operator for points resampling and surface reconstruction. This LOP operator works well when input point sets contain noise or outliers, which is due to the usage of $L_1$ median.
Successively, an improved weighted LOP (WLOP) was proposed to better solve the nonuniform point density problem~\cite{huang2009consolidation}.
Even though these approaches do not rely on normal information as a part of input, they still have assumption that the underlying surface is smooth and tend to fail under severe noise or undersampling.
Huang et al.~\cite{huang2013edge} introduced an edge-aware point set resampling method by resampling away from edges first and then approaching edges or corners progressively.
Although promising results could be generated by this approach, the accuracy of initial normal orientation has a big effect on the outcome.
It is worth mentioning that Wu et al.~\cite{wu2015deep} proposed a deep points representation method to fuse consolidation and completion into one coherent step.
However, since the main focus of that approach is to fill in large holes, no global smoothness is enforced so that this method cannot resist to large noise.

\para{Deep learning-based approaches for point cloud processing} \ \ \ Impressed by the promising performance of deep learning approach to solve image or video related issues, more and more researchers attempt to solve geometry tasks based on such end-to-end framework.
Point clouds, as a direct output of scanning devices, have drawn lots of attention recently since they only contains points without topology information and thus are easier for network to learn from.
\cite{qi2016pointnet,qi2017pointnet++} are the pioneers applying deep learning network on point clouds for classification and segmentation, especially the PointNet++ network that employs a hierarchical feature learning architecture to capture both local and global information.
Fan et al.~\cite{fan2016point} proposed a generation network using encoder and predictor to output point sets from a single image.
Consequently, Lin et al.~\cite{lin2017learning} presented another generation network for 3D object reconstruction from a single image by introducing a pseudo-renderer to produce novel depth maps for loss optimization.s
However, to our knowledge, no work has been done to solve the upsampling task.


